Improving Recommendation Systems with User Personality Inferred from Product Reviews

Personality is a psychological factor that reflects people's preferences, which in turn influences their decision-making. We hypothesize that accurate modeling of users' personalities improves recommendation systems' performance. However, acquiring such personality profiles is both sensitive and expensive. We address this problem by introducing a novel method to automatically extract personality profiles from public product review text. We then design and assess three context-aware recommendation architectures that leverage the profiles to test our hypothesis. Experiments on our two newly contributed personality datasets -- Amazon-beauty and Amazon-music -- validate our hypothesis, showing performance boosts of 3--28%.Our analysis uncovers that varying personality types contribute differently to recommendation performance: open and extroverted personalities are most helpful in music recommendation, while a conscientious personality is most helpful in beauty product recommendation.

==> revision.tex <==
1. Personality distribution figure-merge together
2. Tables 4 and 5-merge together
3. shrink pages
4. add more references  

%TODO: Merge Figures 3 and 4 as top and bottom row.
%TODO: Review Texts column looks off. 
%TODO: Fig 2, move "Score" below so width is more managed outside of the center margin
%TODO: Fig 1. Reformat directly into the tex.  
%TODO: Standardize table format (Table 1 and 2 look different)
%TODO: 2.1.x drop these paragraphs headers and just enumerate it
%TODO: Edit Widows / Orphans
%shrink less than 25% lines, lines 487-492

%highlight editing paragraph with \lxy: shorter, better?
% expand paragraphs: 

